Sound-Proof: Usable Two-Factor Authentication Based on Ambient Sound

Two-factor authentication protects online accounts even if passwords are leaked. Most users, however, prefer password-only authentication. One reason why two-factor authentication is so unpopular is the extra steps that the user must complete in order to log in. Currently deployed two-factor authentication mechanisms require the user to interact with his phone to, for example, copy a verification code to the browser. Two-factor authentication schemes that eliminate user-phone interaction exist, but require additional software to be deployed. In this paper we propose Sound-Proof, a usable and deployable two-factor authentication mechanism. Sound-Proof does not require interaction between the user and his phone. In Sound-Proof the second authentication factor is the proximity of the user's phone to the device being used to log in. The proximity of the two devices is verified by comparing the ambient noise recorded by their microphones. Audio recording and comparison are transparent to the user, so that the user experience is similar to the one of password-only authentication. Sound-Proof can be easily deployed as it works with current phones and major browsers without plugins. We build a prototype for both Android and iOS. We provide empirical evidence that ambient noise is a robust discriminant to determine the proximity of two devices both indoors and outdoors, and even if the phone is in a pocket or purse. We conduct a user study designed to compare the perceived usability of Sound-Proof with Google 2-Step Verification. Participants ranked Sound-Proof as more usable and the majority would be willing to use Sound-Proof even for scenarios in which two-factor authentication is optional.

==> secanalysis.tex <==
\section{Security Analysis}
\label{sec:secanalysis}

Our 2FA mechanism protects against impersonation attacks even if the adversary has the password of a victim user.
Assume the adversary attempts to log in as the victim user at time $t_1$.
Also assume that, at time $t_2$, the phone is notified by the server about the login attempt and starts recording the noise in the environment via its microphone.
Let $p(n)$ be the sample recorded by the phone and assume the phone records up to time $t_3$.
Let $a(n)$ denote the sample submitted by the adversary's computer to the server and assume $a(n)$ is time-stamped from $t_4$ to $t_5$.
Finally assume that $fs$ is the sampling frequency of both recordings.
To succeed in the impersonation attack, the average power of both signals must be above $\tau_C$ and $a(n-l)$ must be highly correlated with $p(n)$ with a maximum lag of $\ell_{max}$.
That is the two samples must satisfy $Pwr(p(n))>\tau_{dB}$, $Pwr(a(n))>\tau_{dB}$ and $\hat{r}_{p,a}(l)>\tau_C$ with $l\in[\pm\ell_{max}*fs]$.




Quantifying the entropy of ambient noise, and hence the likelihood of the adversary guessing the signal recorded by the victim's phone, is a challenging task.
Results are dependent on the environment, the language spoken by the user of the user, gender or age to cite a few~\cite{xxx}.



